A graph-theoretic condition for delay stability of reaction systems

Delay mass-action systems provide a model of chemical kinetics when past states influence the current dynamics. In this work, we provide a graph-theoretic condition for delay stability, i.e., linear stability independent of both rate constants and delay parameters. In particular, the result applies when the system has no delay, implying asymptotic stability for the ODE system. The graph-theoretic condition is about cycles in the directed species-reaction graph of the network, which encodes how different species in the system interact.

==> LineNoPackageOptions.tex <==
%% ##### OPTION FOR LINENO PACKAGE #####
\usepackage[mathlines]{lineno}
    \runninglinenumbers 
        \newcommand*\patchAmsMathEnvironmentForLineno[1]{%
       \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
       \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
       \renewenvironment{#1}%
          {\linenomath\csname old#1\endcsname}%
          {\csname oldend#1\endcsname\endlinenomath}}% 
    \newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
       \patchAmsMathEnvironmentForLineno{#1}%
       \patchAmsMathEnvironmentForLineno{#1*}}%
    \AtBeginDocument{%
    \patchBothAmsMathEnvironmentsForLineno{equation}%
    \patchBothAmsMathEnvironmentsForLineno{align}%
    \patchBothAmsMathEnvironmentsForLineno{flalign}%
    \patchBothAmsMathEnvironmentsForLineno{alignat}%
    \patchBothAmsMathEnvironmentsForLineno{gather}%
    \patchBothAmsMathEnvironmentsForLineno{multline}%
    }
    % end of line number options
